MMP for algebraically integrable foliations

We show that termination of flips for $\mathbb Q$-factorial klt pairs in dimension $r$ implies existence of minimal models for algebraically integrable foliations of rank $r$ with log canonical singularities over a $\mathbb Q$-factorial klt projective variety.

==> Section4.tex <==
%!TeX root=main.tex


\section{Bounding singularities of the algebraic part of a foliation}
\subsection{Family of leaves of an algebraically integrable foliation}


Let $X$ be a normal projective variety and let 
$\mathcal F$ be an algebraically integrable foliation
on $X$.  The following construction follows from \cite[Lemma 3.2]{AD13}:

\begin{construction}
\label{c_fam} There exists a closed subvariety $Z \subset {\rm Chow}(X)$
whose general point parametrises the closure of a leaf of $X$.
Let $p_X\colon X\times Z \rightarrow X$ and $p_Z \colon X \times Z \rightarrow Z$
be the two projections.

If we let $\widehat{X} \subset X \times Z$ to be the universal cycle, then  we have
\begin{enumerate}
\item a birational morphism $\beta\colon \widehat{X} \rightarrow X$ given by 
the restriction of $p_X$ to $\widehat{X}$;

\item 
an equidimensional  contraction
 $f\colon \widehat{X} \rightarrow Z$ given by 
the restriction of $p_Z$ to $\widehat{X}$; and 

\item a foliation $\widehat{\mathcal F} \coloneqq \beta^{-1}\mathcal F$, which is induced by 
$f$.
\end{enumerate}
\end{construction}





\begin{lemma}
\label{lem_neg_disc}
Set up as above. Suppose
that $K_{\mathcal F}$ is $\mathbb Q$-Cartier.  

Then
we may write $K_{\widehat{\mathcal F}}+F \sim_{\mathbb Q} \beta^*K_{\mathcal F}$ where $F \geq 0$
is $\beta$-exceptional.
Moreover, if $E$ is a $\beta$-exceptional divisor which is not $\widehat{\mathcal F}$-invariant
then $E$ is contained in $\Supp F$.
\end{lemma}
\begin{proof}
This is 
\cite[Section 3.6]{Druel21} 
%\cite[Lemma 4.13]{Druel21} 
and \cite[Proposition 4.17]{Druel21}
\end{proof}

 


\begin{lemma}
\label{lem_pure}
Set up as above. Suppose
that $K_{\mathcal F}$ is $\mathbb Q$-Cartier.
Let $E$ be a $\beta$-exceptional divisor.

Then $E$ is not $\widehat{\mathcal F}$-invariant 
if and only if $\beta(E) \subset \Sing \mathcal F$.
\end{lemma}
\begin{proof}
Given a finite cover $X' \rightarrow X$ which is quasi-\'etale around the general point of the centre of $E$ on $X$, let 
\begin{enumerate}
\item $\widehat{X}'$ be the normalisation of $\widehat{X}\times_XX'$;
\item $\widehat{X}' \rightarrow Z'$ be the Stein factorisation of 
$\widehat{X}' \rightarrow Z$; 
\item  $E'$ be 
the preimage of $E$ on $\widehat{X}'$; and
\item  $\mathcal F'$ be the foliation induced by $\mathcal F$ on $X'$.
\end{enumerate}

Note that $E$ is $\cal F$-invariant if and only if $E'$ is $\cal F'$-invariant 
and
\cite[Corollary 5.14]{Druel21} implies that the centre of $E$ is contained 
in $\Sing \mathcal F$ if and only if the centre of $E'$
is contained in $\Sing \mathcal F'$.

Thus, by taking the degree one cover $X'\rightarrow X$ for $K_{\cal F}$ around the general point of the centre of $E$ on $X$, we may freely replace $X$ by $X'$ and we may therefore assume that $K_{\mathcal F}$ is Cartier.
%By taking hyperplane cuts (e.g. see the proof of 
%\cite[Proposition 4.17]{Druel21}),
%we may reduce to the case where $\mathcal F$ is of rank equal to one.\footnote{P: Do we use below the fact that $\cal F$ has rank=1?}

\medskip

If $\beta(E)$ is not contained in $\Sing \cal F$ then  \cite[Lemma 5.9]{Druel21} implies that $\mathcal F$ has canonical singularities around the general point of $\beta(E)$. Thus, by 
Lemma \ref{lem_neg_disc}, it follows that $E$ is  $\widehat{\mathcal F}$-invariant.

Suppose now that $E$ is $\widehat{\mathcal F}$-invariant.
Let $F$ be a general fibre of the induced morphism $E \rightarrow f(E)$. 
By definition of $\beta$ we know that $\beta\vert_F$ is 
a closed immersion. 
 Since $\widehat{\mathcal F}$ is induced by the contraction
$\widehat{X} \rightarrow Z$ it follows that $\widehat{\mathcal F}$
is non-singular at the generic point of any component of a fibre and, in
particular, it is non-singular at the generic point of $F$.
Let $\tilde{\mathcal F}$ be the foliation on $X\times Z$
whose tangent sheaf is $p_X^*T_{\mathcal F}$.
By construction, $\widehat{X}$ is 
$\tilde{\mathcal F}$-invariant  and the restriction of $\tilde{\mathcal F}$
to $\widehat{X}$ is $\widehat{\mathcal F}$.  In particular, 
it follows that $\tilde{\mathcal F}$ is non-singular
at the generic point of $F$ and so $\mathcal F$
is non-singular at the generic point of $\beta(F)$ as required.
\end{proof}

\begin{remark}
\label{rmk_pure} Using the same set-up as above, Lemma \ref{lem_pure} implies that if $F$ is the $\beta$-exceptional divisor as in Lemma \ref{lem_neg_disc}
and if we write $F = F_1+F_0$ where the components of $F_1$ are not $\widehat{\mathcal F}$-invariant and the components of $F_0$ are $\widehat{\mathcal F}$-invariant
then the centres of the irreducible components of 
$F_1$ on $X$ and the centres of the irreducible components of $F_0$ on $X$
are distinct.
\end{remark}


\subsection{A singularity bound}



\begin{proposition}
\label{prop_comparison}
Let  $f\colon X \rightarrow Z$ be an equidimesional 
contraction between normal varieties
and let $\mathcal F$ and $\mathcal G$ be foliations on $X$ and  $Z$ respectively such that 
$df( T_{\mathcal F} )= f^* T_{\mathcal G}$ 
at the generic point of $Z$.
%\footnote{P: is this true everywhere or at the general point of $Z$?}.
Let $\mathcal H$ be the foliation given by $T_{\mathcal F}\cap T_{X/Z}$.

Then $K_{\mathcal H} = (K_{\mathcal F}-f^*K_{\mathcal G})-R(f)_{{\rm n-inv}}$, where $R(f)_{{\rm n-inv}}$ denotes the part of $R(f)$ which is not $\cal F$-invariant. 
\end{proposition}
\begin{proof}
The desired equality may be checked away from a subset of codimension at least two and so, without loss of generality,
we may assume that $X, Z, \mathcal F, \mathcal G$ and $\mathcal H$
are smooth.

We have an exact sequence of vector bundles 
\[
0 \rightarrow T_{\mathcal H} \rightarrow T_{\mathcal F} \xrightarrow{df} f^*T_{\mathcal G},
\]
where $df$ is surjective at the generic point of $Z$. Thus, 
$K_{\mathcal H} = K_{\mathcal F}-f^*K_{\mathcal G}+C$ where $C$ is a vertical divisor.  To prove our claim
it therefore suffices to check locally around a point $x \in X$. Let $n$ and $k$ be the dimension of $X$ and $Z$ respectively. Then there exists a positive integer $m$ such that, in suitable coordinate, $f$ is given by $(x_1, \dots, x_n) \mapsto (x_1^m, \dots, x_k)$.
It follows that $df$ drops rank along $\{x_1 = 0\}$ if and only if $\partial/\partial x_1$ is a local section
of $T_{\mathcal F}$ and our claim follows.
\end{proof}




\begin{corollary}
\label{cor_foliation_is_moduli_part}
Let  $f\colon X \rightarrow Z$ be an equidimesional 
contraction between normal varieties
and let $\mathcal F$ and $\mathcal G$ be foliations on $X$ and  $Z$ respectively such that 
$df(T_{\mathcal F}) = T_{\mathcal G}$ at the generic point of $Z$. 
Suppose that $B$ is a $\mathbb Q$-divisor on $X$ such that $(X/Z, B)$ satisfies Property $(*)$ and let $B_Z$ be the discriminant of the pair $(X/Z,B)$.

Then $(K_{\mathcal F}+B) - f^*(K_{\mathcal G}+B_Z) = K_{\mathcal H}+B^h$. 
\end{corollary}
\begin{proof}
This follows by arguing as in \cite[Proposition 3.6]{ACSS}.
\end{proof}


\begin{corollary}
\label{cor_compar_alg_part}
Let  $f\colon X \rightarrow Z$ be an equidimesional 
contraction between normal varieties
and let $\mathcal F$ and $\mathcal G$ be foliations on $X$ and  $Z$ respectively such that 
$df(T_{\mathcal F}) = T_{\mathcal G}$. Suppose that $T_{X/Z} \subset T_{\mathcal F}$.  

Then $K_{\mathcal F} - f^*K_{\mathcal G} = K_{X/Z}-R(f)_{{\rm inv}}$.
\end{corollary}
\begin{proof}
This follows from Proposition \ref{prop_comparison} and the equality $K_{\mathcal H} = K_{X/Z}-R(f)$,
where $\mathcal H=T_{X/Z}$.
% is foliation induced by $X \rightarrow Z$.
\end{proof}


%The following proposition should be compared with \cite[Proposition 1.8]{Druel15b}

\begin{lemma}
\label{lem_ram_restriction}
Let $(X/Z, B) \rightarrow Z$ be a GLC pair satisfying Property $(*)$ such that the induced morphism $f\colon X\to Z$ is an equidimensional contraction. 
Assume that $(X, B)$ is dlt and that $E$ is a normal irreducible divisor with $m_EB = 1$ and
such that
$h\colon E \rightarrow Z$ is an equidimensional contraction.

Then $R(f)\vert_E = R(h)$.
\end{lemma}
\begin{proof}
%It is easy to see that $R(f)\vert_E \leq R(h)$.  We now show the opposite inequality. 
%Let $D \subset Z$ be any reduced divisor and write $f^*D= \sum a_iF_i$
%and $h^*D = \sum b_iF'_i$ where $F'_i= F_i \cap E$.\footnote{P: is this right, in general? }
Let $\Sigma_Z \subset Z$ be the reduced divisor associated to $(X/Z, B)$.
Then, if we write $(K_X+B)\vert_E = K_E+B_E$, it follows easily that  $(E/Z, B_E)$ admits Property $(*)$ with associated reduced divisor $\Sigma_Z$.


Let $D\subset Z$ be a prime divisor. If  $D$ is not contained in $\Sigma$ then by definition of Property $(*)$ it follows that both $f^*D$ and $h^*D$ are reduced and, in particular, $D$ is not contained in $f(\Supp R(f))$ nor $h(\Supp R(h))$. 

 Now suppose that $D$ is a component of $\Sigma$. 
Then, $f^{-1}(D) \leq B$ and $h^{-1}(D)\leq B_E$. 
Since $(X, B)$ is dlt, it follows that $f^{-1}(D)\vert_E = h^{-1}(D)$. We naturally have
$(f^*D)\vert_E = h^*D$. Thus, our claim follows.
\end{proof}


\begin{proposition}
\label{prop_alg_almost_hol}
Let $X$ be a normal projective variety and let $\mathcal F$ be a foliation with log canonical 
singularities.  Suppose in addition that $a(E, \mathcal F)>-1$ whenever $\epsilon(E) = 1$ ( e.g. $\mathcal F$ has canonical or F-dlt singularities).

Then the algebraic part of $\mathcal F$ is non-dicritical.
\end{proposition}
\begin{proof}
Denote by $\mathcal H$ the algebraic part of $\mathcal F$, and suppose that it is induced by a rational map
$f\colon X \dashrightarrow Z$.  Suppose for sake of contradiction that $f$ is not almost holomorphic.  

Let $\mu\colon \overline X \rightarrow X$ be a Property $(*)$ modification of $\mathcal H$, 
set $\overline{\mathcal H} \coloneqq \mu^{-1}\mathcal H$ and let $\bar{f} \colon \overline{X} \rightarrow \overline{Z}$
be the equidimensional fibration which induces $\overline{\mathcal H}$.  
Moreover, there exists a purely
transcendental foliation $\overline{\mathcal G}$ on $\overline{Z}$ such that 
$\overline{\mathcal F} = \bar{f}^{-1}\overline{\mathcal G}$, 
where $\overline{\mathcal F} = \mu^{-1}\mathcal F$.
Perhaps replacing $\overline{X}$ by a higher model we may assume that 
we have a morphism $\rho\colon \overline{X}\rightarrow \widehat{X}$
where 
$\beta\colon \widehat{X} \rightarrow X$ is the morphism guaranteed 
to exist by Construction \ref{c_fam}. 

Let $\{E_i\}$ denote the collection of $\mu$-exceptional divisors and 
set $\epsilon_i \coloneqq \epsilon(E_i)$.
Since $f$ is not almost holomorphic, there exists a $\mu$-exceptional 
divisor which dominates $\overline{Z}$.
Let $E$ be one such divisor.  
Since $E$ dominates $\overline{Z}$, it is neither $\overline{\mathcal H}$ 
nor $\overline{\mathcal F}$-invariant.

Denote by $h$ the restriction of $\bar{f}$ to $E$, and $\mathcal F_E$ 
(resp. $\mathcal H_E$) the 
restriction of $\overline{\mathcal F}$ (resp. $\overline{\mathcal H}$)
to $E$.  Observe that $\mathcal F_E = h^{-1}\overline{\mathcal G}$ and so 
$\mathcal H_E$ is the algebraic part of $\mathcal F_E$.
Perhaps replacing $\overline X$ by a higher model, we may assume in addition that 
$h\colon E \rightarrow \overline{Z}$ 
is equidimensional. \footnote{P: is this property preserved by the MMP? 
C: I think so, this is \cite[Proposition 2.18]{ACSS}, right? Maybe I'm missing something. P: I still can't see why the MMP induces an MMP for $E$.}


We may write
\[K_{\overline{\mathcal F}}+\sum a_iE_i  = \mu^*K_{\mathcal F}+F\]
where $a_i\leq 0$ if $\epsilon_i = 0$ and $a_i <1$ if $\epsilon_i = 1$
%\footnote{P: I think that instead of $E$, we have a 
%linear combination of the $E_i$ with coefficients $<1$}
and
\[K_{\overline{\mathcal H}}+\sum \epsilon_iE_i  = \mu^*K_{\mathcal H} - G\]
where $F, G \geq 0$ are $\mu$-exceptional.
%Next, since $(\overline{\mathcal H}, \sum \epsilon_iE_i)$ 
%\footnote{P: I think that here, instead of $E$, we should write the sum of 
%all the non-invariant exceptional divisors?} 
%satisfies Property $(*)$, we may run a $(K_{\overline{\mathcal H}}+E)$-MMP over $X$.
By construction of a Property $(*)$ modification we see that 
%By replacing $\overline{X}$ by the output of this MMP we may freely assume that 
$K_{\overline{\mathcal H}}+\sum \epsilon_iE_i$ is $\mu$-nef.


By Proposition \ref{prop_comparison} we have 
\[K_{\overline{\mathcal H}}+\bar{f}^*K_{\overline{\mathcal G}}+R(\bar{f})_{{\rm n-inv}} = K_{\overline{\mathcal F}}\]
and
\[K_{\mathcal H_E}+h^*K_{\overline{\mathcal G}}+R(h)_{{\rm n-inv}} = K_{\mathcal F_E}.\]

By adjunction for algebraically integrable foliations, 
\cite[Proposition 3.2]{ACSS}, we may write 
$(K_{\overline{\mathcal H}}+\sum \epsilon_iE_i)\vert_E = K_{\mathcal H_E}+\Delta_E$
where $\Delta_E \geq 0$. 
Since $(\overline{\mathcal H}, \sum \epsilon_iE_i)$ satisfies Property $(*)$,  
Lemma \ref{lem_ram_restriction} 
\footnote{P: do we know that $(\overline X,G)$ is dlt? here $G$ is the divisor associated to $(\overline H,\sum \epsilon(E_i)E_i)$}
implies that $R(\bar{f})\vert_E = R(h)$, and so 
it follows that we may write 
$(K_{\overline{\mathcal F}}+\sum \epsilon_iE_i)\vert_E = K_{\mathcal F_E}+\Delta'_E$
where $\Delta'_E = \Delta_E$.
%\footnote{P: maybe I am doing something wrong here, but I get the opposite inequality. 
%C: Yes, I think you're right, that was my stupid mistake.  However, I think since 
%$(\mathcal H, E)$ admits Property $(*)$ we actually get an equality $R(h) = R(f)\vert_E$.}

By construction of the Property $(*)$-modification we know that 
$K_{\mathcal H_E}+\Delta_E$ is $\mu$-nef.
By Proposition \ref{prop_comparison} we have 
$K_{\mathcal H_E}+h^*K_{\overline{\mathcal G}}+R(h)_{{\rm n-inv}} = K_{\mathcal F_E}$.
Since $\overline{\mathcal G}$ is purely transcendental it follows by \cite{CP19} that $K_{\overline{\mathcal G}}$
is pseudo-effective.  It follows that $K_{\mathcal F_E}+\Delta_E$ is $\mu$-pseudoeffective.

Let $c_X(E)$ be the centre of $E$ on $X$.  By Remark \ref{rmk_pure}
up to shrinking $X$ about $c_X(E)$ 
we may assume 
that every $\beta$-exceptional divisor is not invariant.  In particular, 
we see that $\rho_*(K_{\overline{\mathcal F}}+\sum \epsilon_iE_i) = 
K_{\widehat{\mathcal F}}+\sum \rho_*E_i$ is $\beta$-pseudoeffective.
However, by Lemma \ref{l_exceptional} it cannot be the case that 
$K_{\widehat{\mathcal F}}+\sum \rho_*E_i$ is $\beta$-pseudoeffective, a contradiction.
%
%On the other hand, by Lemma \ref{l_exceptional} $K_{\mathcal F_E}+\Delta'_E$ 
%is not $\mu$-pseudoeffective, a contradiction.
%\footnote{P: why?}
\end{proof}


\begin{corollary}
Let $X$ be a normal projective variety and let $\mathcal F$ be a foliation with log canonical 
singularities.  Suppose in addition that $a(E, \mathcal F)>-1$ whenever $\epsilon(E) = 1$ (e.g., $\mathcal F$ has canonical or F-dlt singularities).
Suppose that $-K_{\mathcal F}$ is nef and is not numerically trivial.

Then the algebraic part of $\mathcal F$ is induced by an equidimensional fibration.
\end{corollary}
\begin{proof}
By \cite{CP19} the algebraic part of $\mathcal F$, call it $\mathcal H$, is non-trivial, and by 
Proposition \ref{prop_alg_almost_hol} $\mathcal H$ is induced by an almost holomorphic map.
Following the proof of \cite[Claim 4.3]{MR3935068} we see that $K_{\mathcal F} \equiv K_{\mathcal H}$.
%We remark that smoothness of $X$ is not needed here.\footnote{C: note to self, double check this}
%We next claim that $K_{\mathcal H}$ is weakly regular.
%This will follow by adapting the proof of \cite[Proposition 3.1]{MR3935068}
%to the singular case.
The result then follows by \cite[Corollary 1.4]{Ou21}.
\iffalse
\footnote{P: Where is this proven in Ou? 
can't $\cal G$ in Ou's main theorem be something different from the zero foliation?
C: I updated the reference, but you're right a bit more needs to be said.  In the statement of the corollary
Ou requires the fibres
to be rationally connected to get locally trivial, although I think his proof can be slightly modified
to get around this.  I've updated the statment of the corollary to reflect the weaker result, but I'll think
more about making the stronger version work.}
\fi 
\end{proof}






%\begin{proposition}
%\label{prop_alg_almost_hol}
%Let $X$ be a normal projective variety and let $\mathcal F$ be 
%a foliation with log canonical 
%singularities.  Suppose in addition that $a(E, \mathcal F)>-1$ 
%whenever $\epsilon(E) = 1$ 
%( e.g. $\mathcal F$ has canonical or F-dlt singularities).
%
%Then the algebraic part of $\mathcal F$ is non-dicritical.
%\end{proposition}
%\begin{proof}
%Suppose for sake of contradicition that $\mathcal F$ is dicritical.
%Let $\mathcal H$ be the algebraic part of $\mathcal F$
%and let
% \begin{center}
%\begin{tikzcd}
%\overline{X} \arrow[r, "\mu"] \arrow[d, "f"] & X \\
%Z &
%\end{tikzcd}
%\end{center}
%be the model guaranteed by 
%Construction \ref{c_fam} applied to $\mathcal H$.
%By assumption there exists a purely transcendtal foliation $\mathcal G$
%on $Z$ such that $f^{-1}\mathcal G = \mu^{-1}\mathcal F$.
%
%Let $E$ be an irreducible $\mu$-exceptional divisor which is not $\overline{\mathcal H}$
%invariant (using notation as in Construction \ref{c_fam}).
%
%Let $\mathcal H_E$ be the restriction of $\overline{\mathcal H}$ to $E$
%and let $\mathcal F_E$ be the restiction of $\mu^{-1}\mathcal F$ to $E$.
%
%
%
%
%
%\end{proof}



%\iffalse
%We now prove a base point free theorem for algebraically integrable foliations. 
%\begin{theorem}
%Let $X$ be a normal projective variety, let $\mathcal F$ be an algebraically integrable foliation on $X$
%and let $\Delta \geq 0$ be a $\mathbb Q$-divisor so that $(\mathcal F, \Delta)$ has F-dlt singularities
%and $(X, \Delta)$ is klt. Let $A$ be an ample $\mathbb Q$-divisor on $X$ such that $L=K_{\cal F}+\Delta+A$ is a nef $\mathbb Q$-divisor. 
%
%Then $L$ is semi-ample. 
%\end{theorem}
%\fi



%
%
%\iffalse
%\begin{proof}
%By \cite[Theorem 3.9]{ACSS} there exists a supporting hyperplane $H_R$ to $R$.  We may write
%$H_R = K_{\mathcal F}+\Delta+A$ where $A$ is ample.  Either (i) $H_R$ is big or (ii) it is not.
%Let us first assume that we are in case (i).
%
%\medskip
%
%Let $\pi\colon \overline{X} \rightarrow X$ be a Property $(*)$ modification
%of $(\mathcal F, \Delta)$, which is guaranteed to exist by 
%\cite[Theorem 3.10]{ACSS}, and let $B \ge 0$ be the associated invariant divisor.
%%Suppose moreover that $\overline{\mathcal F}\coloneqq \pi^{-1}\mathcal F$
%%is induced by a fibration $f\colon \overline{X} \rightarrow Z$.  
%Write $K_{\overline{\mathcal F}}+\overline{\Delta} = \pi^*(K_{\mathcal F}+\Delta)$ 
%and by Lemma \ref{lem_discrep} we may write $K_{\overline{X}}+\overline{\Delta}+E = \pi^*(K_X+\Delta)+F$
%where $F \ge 0$ and $\lfloor \overline{\Delta}+E \rfloor = 0$.
%
%Since $(\mathcal F, \Delta)$ is F-dlt it follows that $\Exc \pi$ is $\overline{\mathcal F}$-invariant.
%
%
%%Let $\phi\colon \overline{X} \dashrightarrow Y$ be a $K_{\overline{\mathcal F}}+\overline{\Delta}$-MMP,
%%which exists since $(\overline{\mathcal F}, \overline{\Delta})$ has Property $(*)$.
%%Indeed, following \cite[Lemma 3.14]{ACSS} we can run a 
%%$K_{\overline{\mathcal F}}+\overline{\Delta}$-MMP by running a 
%%$K_{\overline{X}}+\overline{\Delta}+B$-MMP. 
%
%
%
%Since $X$ is $\mathbb Q$-factorial we may find
%a $\pi$-exceptional divisor $G \ge 0$ such that $-G$ is $\pi$-ample.
%
%Fix $\epsilon>0$ sufficiently small so that 
%\begin{enumerate}
%\item each step in the MMP given by 
%$\phi\colon \overline{X} \dashrightarrow Y$, is 
%$(K_{\overline{\mathcal F}}+\overline{\Delta})+\epsilon (K_{\overline{X}}+\overline{\Delta}+E)$-negative;
%
%
%\item $\epsilon < \frac{1}{4\dim X m_1m_2}$ where
%$m_1$ is the Cartier index of $H_R$, $m_2$ is the least common multiple of the Cartier index of 
%$\rho_*(K_{\overline{\mathcal F}}+\overline{\Delta})$ where $\rho\colon \overline{X} \rightarrow Y$
%is any $K_{\overline{\mathcal F}}+\overline{\Delta}$-negative contraction which is $\pi^*H_R$-trivial
%(by finiteness of models, 
%Proposition \ref{prop_finiteness_of_models},
%there are only finitely many such contractions and so $m_2$ is finite); and
%
% 
%\item $A-\epsilon (K_X+\Delta)$ is ample.
%\end{enumerate}
%%Since any two minimal models of $(\mathcal F, \Delta)$ can be related by a sequence
%%of flops we see that $m_2$ is independent of our choice of $\phi$.
%
%
%Fix $\delta>0$ sufficiently small so that we have 
%$H\coloneqq \pi^*(A - \epsilon (K_X+\Delta))-\delta G$ is ample and 
%$(\overline{X}, \overline{\Delta} + E+\frac{\delta}{\epsilon}G)$ is klt.
%Observe that we may write
%\[
%\pi^*H_R+\epsilon F \sim (K_{\overline{\mathcal F}}+\overline{\Delta}+\frac{1}{1+\epsilon}H)
%+\epsilon (K_{\overline{X}}+\overline{\Delta}+E+\frac{1}{1+\epsilon}H+\frac{\delta}{\epsilon} G).
%\]
%
%
%%By Proposition \ref{prop_adjoint_*_MMP} 
%We claim that  may run an adjoint MMP for 
%$K\coloneqq (K_{\overline{\mathcal F}}+\overline{\Delta}+\frac{1}{1+\epsilon}H)
%+\epsilon (K_{\overline{X}}+\overline{\Delta}+E+\frac{1}{1+\epsilon}H+\frac{\delta}{\epsilon} G)$
%with scaling of $H$.  We explain how to run this MMP now.
%
%
%
%%moreover, we may take this MMP to be an MMP with scaling of $H$.  
%%Thus, each step in this MMP is in fact a step in an adjoint MMP for  
%%$K\coloneqq (K_{\overline{\mathcal F}}+\overline{\Delta})
%%+\epsilon (K_{\overline{X}}+\overline{\Delta}+E+\frac{\delta}{\epsilon} G)$.
%
%Let $\phi \colon \overline{X} \dashrightarrow \overline{X}_1$ be an MMP for 
%$K_{\overline{\mathcal F}}+\overline{\Delta}+\frac{1}{1+\epsilon}H$
%with scaling of $H$.  Indeed, following \cite[Lemma 3.14]{ACSS} we can run a 
%$K_{\overline{\mathcal F}}+\overline{\Delta}+\frac{1}{1+\epsilon}H$-MMP with scaling of $H$ by running a 
%$K_{\overline{X}}+\overline{\Delta}+B+\frac{1}{1+\epsilon}H$-MMP with scaling of $H$.
%By finiteness of models, \cite[Theorem E]{BCHM06} by perhaps replacing $\epsilon$ by a smaller value, 
%we may assume that each
%step in this MMP is $K$-negative as well.
%
%
%Next, consider a sequence of steps in a 
%$K_{\overline{X}_1}+\phi_*(\overline{\Delta}+E+\frac{1}{1+\epsilon}H+\frac{\delta}{\epsilon} G)$-MMP
%with scaling of $\phi_*H$ which only contracts $\phi_*K$-negative extremal rays.
%
%
%Call the steps of this MMP $(Y_i, \mathcal G_i, A_i, D_i, \Theta_i)$
%where $Y_0 \coloneqq \overline{X}_1$, $\mathcal G_0 = \phi_*\overline{\mathcal F}$, $A_0 = \phi_*H$,
%$D_0 = \phi_*(\overline{\Delta}+E+\frac{1}{1+\epsilon}H+\frac{\delta}{\epsilon} G)$ and 
%$\Theta_0 = \phi_*\overline{\Delta}$.
%Note that $D_{i, {\rm n-inv}} = \Theta_i+\frac{1}{1+\epsilon} A_i$.
%
%
%Let each step $\psi_i\colon Y_i \dashrightarrow Y_{i+1}$ contract or flip an extremal ray $R_i$
%which is both $K_{Y_i}+D_i$-negative and $(K_{\mathcal G_i}+D_{i, {\rm n-inv}})+\epsilon (K_{Y_i}+D_i)$-negative.
%
%
%We claim that $R_i$ is also $K_{\mathcal G_i}+\Theta_i$-non-positive.  We argue by induction on $i$.
%Indeed, by the inductive assumption $\overline{X} \dashrightarrow Y_i$ is a 
%$K_{\overline{\mathcal F}}+\overline{\Delta}$-negative contraction, and so the Cartier index of
%$K_{\mathcal G_i}+\Theta_i$ divides $m_2$.  
%
%Next, choose a curve $\xi_i$ such that $R_i = \mathbb R_{+}[\xi_i]$ and such that 
%$-(K_{Y_i}+D_i)\cdot \xi_i \leq 2\dim X$ and suppose for sake
%of contradiction that $(K_{\mathcal G_i}+\Theta_i)\cdot \xi_i>0$.  
%Since $D_{i, {\rm n-inv}} = \Theta_i+\frac{1}{1+\epsilon} A_i$, and since $A_i\cdot \xi_i>0$ by the scaling
%assumption, we see that $(K_{\mathcal G_i}+D_{i, {\rm n-inv}})\cdot \xi \geq \frac{1}{m_2}$.
%It follows that $((K_{\mathcal G_i}+D_{i, {\rm n-inv}})+\epsilon (K_{Y_i}+D_i))\cdot \xi_i \geq 0$, a contradiction.
%
%Finally, observe that since this is an MMP with scaling of a big divisor, this process must terminate.  Let 
%$\psi\colon \overline{X}_1 \dashrightarrow \overline{X}_2$ denote the output of this MMP.
%
%
%By our choice of $\epsilon$ note that we may take each step of $\phi$ and 
%$\psi$ to be $\pi^*H_R$-trivial.
%
%
%
%
%
%
%
%
%%Next, let $\psi\colon \overline{X}_1 \dashrightarrow \overline{X}_2$ be a partial 
%%$K_{\overline{X}_1}+\phi_*(\overline{\Delta}+E+\frac{1}{1+\epsilon}H+\frac{\delta}{\epsilon} G)$-MMP
%%with scaling of $\phi_*H$ which only contracts $\phi_*K$-negative extremal rays.
%%We claim that each contracted ray is 
%
%
%
%
%
%
%
%%Each step of this MMP contracts a ray $\mathbb R_{+}[\xi]$ with $0<-K\cdot \xi \leq 4\dim X$.
%%So by our choice of $\epsilon$ each step of this MMP will be $H_R$-trivial and each step of this MMP
%%will be either $K_{\overline{\mathcal F}}+\overline{\Delta}$-negative or trivial.
%
%%Indeed, up to replacing $\phi$ by a different MMP, we may write this adjoint MMP as a composition
%%$\phi\colon \overline{X} \dashrightarrow Y$ and $\psi\colon Y \dashrightarrow \overline{X}_{m}$,
%%where each step of $\psi$ is $\phi_*(K_{\overline{\mathcal F}}+\overline{\Delta})$-trivial.
%
%
%We have that $\psi_*\phi_*(\pi^*H_R+\epsilon F)$ is nef, and since each step of the MMP is 
%$\pi^*H_R$-trivial, it suffices to show that 
%$\psi_*\phi_*(\pi^*H_R+\epsilon F)$ is semi-ample.
%
%
%Next, each step of this adjoint MMP is either a step
%in a $K_{\overline{X}}+\overline{\Delta}+B$-MMP or a $K_{\overline{X}}+\overline{\Delta}+E$-MMP  
%and so we may write 
%$\phi_*\psi_*(K_{\overline{X}}+\overline{\Delta}+E+\frac{1}{\epsilon}H) \sim K_{\overline{X}_m}+\Theta$
%where $(\overline{X}_m, \Theta)$ is klt.
%
%Finally, observe that 
%$\psi_*\phi_*(\pi^*H_R+\epsilon F) - \epsilon (K_{\overline{X}_m}+\Theta) 
%\sim \psi_*\phi_*(K_{\overline{\mathcal F}}+\overline{\Delta})$ which is nef.  
%We may therefore apply the base point free theorem, \cite[Theorem 3.3]{KM98}, to conclude.
%
%\medskip
%
%Now, in the case where $H_R$ is not big, it is not hard to deduce that in fact
%$R$ is a $K_X+\Delta$-negative extremal ray, in which case we may conclude by
%applying the classical version of the contraction theorem.
%
%
%
%
%\end{proof}
%\fi







%\begin{proof}
%By \cite[Theorem 3.9]{ACSS} there exists a supporting hyperplane $H_R$ to $R$.  We may write
%$H_R = K_{\mathcal F}+\Delta+A$ where $A$ is ample.  Either (i) $H_R$ is big or (ii) it is not.
%Let us first assume that we are in case (i).
%
%Let $\pi\colon \overline{X} \rightarrow X$ be a Property $(*)$ modification
%of $(\mathcal F, \Delta)$, which is guaranteed to exist by 
%\cite[Theorem 3.10]{ACSS}, and suppose moreover that $\overline{\mathcal F}\coloneqq \pi^{-1}\mathcal F$
%is induced by a fibration $f\colon \overline{X} \rightarrow Z$.  Write $K_{\overline{\mathcal F}}+\overline{\Delta} = \pi^*(K_{\mathcal F}+\Delta)$ and
%let $G \geq 0$ be the vertical divisor so that $(\overline{X}/Z, \overline{\Delta}+G)$ has Property $(*)$.
%We may write $(K_{\overline{X}}+\overline{\Delta}+E) = \pi^*(K_X+\Delta+\pi_*G)+F$ where $E, F \geq 0$
%and $\lfloor \overline{\Delta}+E\rfloor=0$.
%
%
%We define $A_{\epsilon}\coloneqq \frac{1}{1+\epsilon}(A-\epsilon(K_X+\Delta))$, 
%so we have $H_R = (K_{\mathcal F}+\Delta+A_{\epsilon})+\epsilon (K_X+\Delta+A_{\epsilon})$.
%Let $0 \leq D_{\epsilon}$ be a general choice of a divisor $\mathbb Q$-linearly equivalent to 
%$\pi^*A_{\epsilon}$.
%
%
%We may write 
%\[
%(K_{\overline{\mathcal F}}+\overline{\Delta}+D_{\epsilon})+
%\epsilon (K_{\overline{X}}+\overline{\Delta}+E+D_{\epsilon}) = \pi^*H_R+\epsilon F).
%\] 
%
%
%Following \cite[Lemma 3.14]{ACSS} we can run a 
%$K_{\overline{\mathcal F}}+\overline{\Delta}+D_{\epsilon}$-MMP by running a 
%$K_{\overline{X}}+\overline{\Delta}+G+D_{\epsilon}$-MMP.  
%By finiteness of models 
%we can deduce that this MMP will be independent of $\epsilon>0$ when $\epsilon$ is sufficiently
%small.  Choose $\eta_0>0$ so that for all $0<\epsilon \leq \eta_0$ this MMP does not depend on $\epsilon$.%
%
%Call this MMP $\varphi\colon \overline{X} \dashrightarrow \overline{X}_1$ and 
%set $\overline{\mathcal F}_1 = \varphi_*\overline{\mathcal F}$, 
%$\overline{\Delta}_1 = \varphi_*\overline{\Delta}$, $D_{\epsilon, 1} = \varphi_*D_{\epsilon}$
%and $E_1 = \varphi_*E$.
%
%We observe that for $\epsilon>0$ sufficiently small that each step of this MMP is also $\pi^*H_R$-trivial.
%
%
%Next, we run a partial $K_{\overline{X}_1}+\overline{\Delta_1}+E_1+D_{\epsilon, 1}$-MMP 
%(which is possible since $(\overline{X}_1, \overline{\Delta_1}+G_1+D_{\epsilon, 1})$ is dlt)
%by only contracting rays along which the strict transform of $\pi^*H_R$ is trivial and
%which are negative for the strict transform of $\pi^*H_R+\epsilon F$, in particular
%each step of this MMP will be negative for the strict transform of $F$.
%Again, for $\epsilon>0$ sufficiently small this will MMP will be independent of $\epsilon$.
%
%
%%, and call this
%%MMP $\psi\colon \overline{X}_1 \dashrightarrow \overline{X}_2$.
%
%Let $\overline{X}_1 \dashrightarrow \overline{X}_2 
%\dashrightarrow \dots \dashrightarrow \overline{X}_m$
%be the steps in this MMP.
%
%
%\begin{claim}
%Let $\psi_i\colon \overline{X}_i \dashrightarrow \overline{X}_{i+1}$ be a step
%in the above MMP.
%Then there exists $\epsilon_0>0$ such that if 
%$0<\epsilon<\epsilon_0$
%
%\begin{enumerate}
%\item $\psi_i$ is
%$K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+D_{\epsilon, i}$-trivial;
%
%\item let $\theta \coloneqq \psi_{m-1}\circ \dots \circ \psi_i \circ \varphi$,
%then $\theta_*(\pi^*H_R+\epsilon F)$ is nef; and
%
%\item  $\theta_*F = 0$.
%\end{enumerate}
%\end{claim}
%\begin{proof}[Proof of Claim]
%We will prove the claim by induction on the number of steps of our MMP.  
%We will first show that items (1), (2) and (3) holds for $\epsilon>0$ sufficiently small
%and
% we will then produce an explicit value of $\epsilon_0$ at the end of the proof of the claim.
%
%We first prove item (1).
%Set $A_1 \coloneqq \varphi_*\pi^*A$ and note that we have 
%$D_{\epsilon, 1} = \frac{1}{1+\epsilon}(A - \epsilon(K_{\overline{X}_1}+
%\overline{\Delta}_1+E_1)+\epsilon F_1)$.
%We have the following equivalences
%\[K_{\overline{\mathcal F}_i}+\overline{\Delta_i}+D_{\epsilon, i} \sim_{\mathbb Q} 
%K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+A_i - \frac{\epsilon}{1+\epsilon}
%(K_{\overline{X}_i}+\overline{\Delta}_i+E_i+A_i-F_i)\]
%and
%\[K_{\overline{X}_i}+\overline{\Delta}_i+E_i+D_{\epsilon, 1} \sim_{\mathbb Q} \frac{1}{1+\epsilon}
%(K_{\overline{X}_i}+\overline{\Delta}_i+E_i+A_i)-\frac{\epsilon}{1+\epsilon} F_i,\]
%where the subscript $i$ denotes the strict transform of the corresponding divisor on $\overline{X}_i$.
%
%
%Let $m_1$ be the Cartier index of $K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1$ and note
%that $K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1$ is nef, by our choice of $\epsilon$.
%We will show that in fact each step of this MMP is
%$K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+A_i$-trivial, which will imply
%by induction that the Cartier index of $K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+A_i$
%is $m_1$.  
%
%
%Let $R_i$ be the $K_{\overline{X}_i}+\overline{\Delta}_i+E_i+D_{\epsilon, i}$-negative extremal ray 
%which is contracted/flipped by $\psi_i$,
%and let $\xi$ be a curve spanning $R_i$ with 
%$-(K_{\overline{X}_i}+\overline{\Delta}_i+E_i+D_{\epsilon, i})\cdot \xi \leq 2\dim X$.%
%
%As noted, $\psi_i$ is $F_i$-negative.
%It follows
%that $(K_{\overline{\mathcal F}_i}+\overline{\Delta_i}+D_{\epsilon, i})\cdot \xi \geq 
%(K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+A_i)\cdot \xi$.  In particular, for 
%$\lambda \geq 2m_1\dim X$ we have 
%every $K_{\overline{X}_i}+E_i+D_{\epsilon, i}+
%\lambda (K_{\overline{X}_i}+\overline{\Delta}_i+E_i+D_{\epsilon, i})$-negative extremal ray is 
%$(K_{\overline{X}_i}+\overline{\Delta}_i+E_i+D_{\epsilon, i})$-trivial and
%is $K_{\overline{\mathcal F}_i}+\overline{\Delta}_i+A_i$-trivial.
%
%\medskip
%
%Now we prove item (2).  Let $m$ be the Cartier index of $\pi^*H_R$. Since each step
%of these MMPs is $\pi^*H_R$ trivial it follows that $m$ is the Cartier index of
%$(\pi^*H_R)_i$ (the strict transform of $\pi^*H_R$ on $\overline{X}_i$).
%Arguing as in the proof of item (1) we see
%that if $R_i$ is $K_{\overline{X}_i}+E_i+D_{\epsilon, i}+\lambda (\pi^*H_R)_i$-negative
%where  $\lambda > 2m\dim X$ then it is $(\pi^*H_R)_i$-trivial.  It follows that 
%$\theta_*((1+\lambda)\pi^*H_R+\epsilon F$, and hence $\theta_*(\pi^*H_R+\frac{\epsilon}{1+\lambda}F)$,
%is nef.
%
%\medskip
%
%Next we prove item (3).
%Observe that $\Supp F = \mathbb B_-(\pi^*H_R+\epsilon F)$ for all $\epsilon>0$.
%Thus, the $\pi^*H_R+\epsilon F$-MMP must contract $\Supp F$, i.e. $\theta_*F = 0$. 
%\medskip




%Finally, our above arguments show that we may take $\epsilon_0 = \frac{1}{4mm_1\dim X}$
%to ensure that for $0<\epsilon<\epsilon_0$ the three items of the claim hold.
%




%\iffalse
%
%We first claim that for $\epsilon>0$ sufficiently small, and up to replacing $\psi$ by some
%partial MMP, we may assume that each step of $\psi$ is 
%$K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+D_{\epsilon, 1}$-trivial and
%that \[\overline{K}_{\epsilon}\coloneqq \psi_*((K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+D_{\epsilon, 1})+\epsilon\psi_*(K_{\overline{X}_1}+\overline{\Delta_1}+D_{\epsilon, 1})\]
%is nef.
%
%Set $A_1 \coloneqq \varphi_*\pi^*A$ and note that we have 
%$D_{\epsilon, 1} = \frac{1}{1+\epsilon}(A - \epsilon(K_{\overline{X}_1}+\overline{\Delta}_1+E_1)+\epsilon F_1)$.
%We have the following equivalences
%%Let $A_1 = \varphi_*\pi^*A$, and note that we have the following equivalences
%\[K_{\overline{\mathcal F}_1}+\overline{\Delta_1}+D_{\epsilon} \sim_{\mathbb Q} 
%K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1 - \frac{\epsilon}{1+\epsilon}(K_{\overline{X}_1}+\overline{\Delta}_1+E_1+A_1-F_1)\]
%and
%\[K_{\overline{X}_1}+\overline{\Delta}_1+E_1+D_{\epsilon, 1} \sim_{\mathbb Q} \frac{1}{1+\epsilon}(K_{\overline{X}_1}+\overline{\Delta}_1+E_1+A_1)-\frac{\epsilon}{1+\epsilon} F_1.\]

%Let $m_1$ be the Cartier index of $K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1$ and note
%that $N\coloneqq K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1$ is nef, by our choice of $\epsilon$.
%Let $R'$ be a $K_{\overline{X}_1}+\overline{\Delta}_1+E_1+D_{\epsilon, 1}$-negative extremal ray
%and let $\xi$ be a curve spanning $R'$ with 
%$-(K_{\overline{X}_1}+\overline{\Delta}_1+E_1+D_{\epsilon, 1})\cdot \xi \leq 2\dim X$.

%We claim that each step of the MMP given by $\varphi$ and $\psi$ is $F$-negative.
%Indeed, each step of $\phi$ and $\psi$ is a step of $\pi^*H_R+\epsilon F$-MMP,
%and since each step of these MMPs are $\pi^*H_R$-trivial, we seethat they are in
%fact $F$-negative.
%
%It follows
%that $(K_{\overline{\mathcal F}_1}+\overline{\Delta_1}+D_{\epsilon})\cdot \xi \geq (K_{\overline{\mathcal F}_1}+\overline{\Delta}_1+A_1)\cdot \xi$.  In particular, for $\lambda \geq 2m_1\dim X$ we have 
%every $K_{\overline{X}_1}+E_1+D_{\epsilon, 1}+\lambda (K_{\overline{X}_1}+\overline{\Delta}_1+E_1+D_{\epsilon, 1})$-negative extremal ray is $(K_{\overline{X}_1}+\overline{\Delta}_1+E_1+D_{\epsilon, 1})$-trivial.
%
%
%Finally, observe $\psi_*\varphi_*F = 0$.%
%
%We next claim that we may write
% $\psi_*(K_{\overline{X}_1}+\overline{\Delta_1}+D_{\epsilon, 1})\sim_{\mathbb Q} K_{\overline{X}_2}+\Theta$
%where $(\overline{X}_2+\Theta)$ is klt.  Indeed, this is a straightforward consequence
%of the fact that $(X, \Delta)$ is klt, induction on the number of steps of the MMP and \cite[Lemma 3.27]{CS18}.
%\footnote{C: sorry I was just a bit lazy in looking for a good reference, I will find a better one}
%%
%
%
%
%We finally claim that for $\epsilon>0$ sufficiently small 
%each step of the MMPs given by $\varphi$ and $\psi$ are 
%in fact $H_R$-trivial.
%Indeed, we may write
%\[\pi^*H_R+\epsilon F = (K_{\overline{F}}+\overline{\Delta}+D_{\epsilon})+
%\epsilon(K_{\overline{X}}+\overline{\Delta}+G+D_{\epsilon})\]
%and we may observe that each step of these MMPs will contract 
%a curve $\xi$ such that $0<-K\cdot \xi \leq 2\dim X$
%where $K$ is the relevant divisor.  It follows that it suffices to contract
%$\pi^*H_R$-trivial curves in order to guarantee that $\overline{K}_{\epsilon}+2m\dim X\psi_*\varphi_*H_R$
%is nef where $m$ is the Cartier index of $H_R$.  
%Next, since $\overline{K}_\epsilon =\psi_*\phi_*(\pi^*H_R+\epsilon F)$
%we have $\overline{K}_{\epsilon}+2\dim X M\psi_*\varphi_*H_R = 
%(1+2m\dim X)\overline{K}_{\frac{\epsilon}{2m\dim X}}$.  Again, by finiteness of models we see
%that for $\epsilon>0$ sufficiently small we may take the above MMPs to be $\pi^*H_R$ trivial.%
%
%\fi
%\end{proof}






%To conclude, 
%we first observe that $(\overline{X}_m, \overline{\Delta}_m+E_m+D_{\epsilon, m})$
%is klt and that 
%that $\theta_*\pi^*H_R$ is big and nef.
%
%We next have 
%\[\frac{1}{\epsilon}(\theta_*\pi^*H_R) - (K_{\overline{X}_m}+\overline{\Delta}_m+E_m+D_{\epsilon, m}) \sim 
%\frac{1}{\epsilon}\theta_*((K_{\overline{\mathcal F}}+\overline{\Delta}+D_{\epsilon})\]
%is nef.  We may apply the classical basepoint free theorem, \cite[Theorem 3.3]{KM98}, to see
%that $\theta_*\pi^*H_R$, and hence $H_R$ is semi-ample.
%
%The morphism given by $|kH_R|$ for $k \gg 0$ is therefore our desired contraction.
%It is then easy to check that it satisfies all our required properties.



%\medskip
%
%Now, in the case where $H_R$ is not big, it is not hard to deduce that in fact
%$R$ is a $K_X+\Delta$-negative extremal ray, in which case we may conclude by
%applying the classical version of the contraction theorem.
%\end{proof}
%
%\iffalse
%\begin{proof}[Proof sketch]
%By \cite[Theorem 3.9]{ACSS} there exists a supporting hyperplane $H_R$ to $R$.
%
%Let $\pi\colon X' \rightarrow X$ be a Property $(*)$ modification of $(\mathcal F, \Delta)$
%which is guaranteed to exist by \cite[Theorem 3.10]{ACSS}, write 
%$K_{\mathcal F'}+\Delta' = \pi^*(K_{\mathcal F}+\Delta)$
%where $\mathcal F' = \pi^{-1}\mathcal F$ and write $K_{X'}+\Gamma = \pi^*(K_X+\Delta)+F$ where $F \geq 0$.
%%Note that all the $\pi$-exceptional divisors are $\mathcal F'$-invariant
%By Lemma \ref{lem_discrep} observe that $\Gamma_{{\rm n-inv}} = \Delta'$.
%
%Let $G \geq 0$ be a $\pi$-exceptional divisor such that $-G$ is $\pi$-ample.
%
%For any $1 \gg \epsilon>0$ we may find an ample divisor $A$ so that
%$H_R = (K_{\mathcal F}+\Delta)+\epsilon (K_X+\Delta)+(1+\epsilon)A$.
%
%We may find an ample divisor $A'$ on $X'$ such that
%$(1+\epsilon)A' \sim (1+\epsilon)\pi^*A-\epsilon\delta G$ where $\delta>0$.
%
%It follows that 
%\[(K_{\mathcal F'}+\Delta'+\pi^*A)+\epsilon (K_{X'}+\Gamma+\pi^*A) 
%\sim_{\mathbb Q} (K_{\mathcal F'}+\Delta'+A')+\epsilon (K_{X'}+\Gamma+\delta G+A').\]
%
%
%By taking $0<\delta\ll 1$, and $H \sim_{\mathbb Q}A'$ to be sufficiently general if
%we set $B = \Gamma+\delta G+H$ then $(\mathcal F', B_{{\rm n-inv}})$ has F-dlt singularities and
%satisfies Property $(*)$
%and $(X', B)$ has klt singularities.
%
%By construction if we set $K_{\epsilon} \coloneqq (K_{\mathcal F'}+B_{{\rm n-inv}}) +\epsilon (K_{X'}+B)$
%then $K_{\epsilon} = \pi^*H_R+\epsilon F$.
%
%Let $M_1$ denote the Cartier index of $K_{\mathcal F'}+B_{{\rm n-inv}}$, so for $0<\epsilon < \frac{1}{2M_1\dim X}$
%we may run a $K_{\epsilon}$-MMP.  Let $M_2$ denote the Cartier index of $H_R$.
%By \cite[Theorem 3.9]{ACSS} and
%\cite[Theorem 3.7]{KM98} we see that there if $\tilde{R}$ is a $K_{\epsilon}$-negative extremal ray
%there is a curve $\xi$ spanning $\tilde{R}$ 
%so that $K_{\epsilon} \cdot \xi \leq 4\dim X$.
%In particular, if $\xi\cdot \pi^*H_R >0$ then $(K_{\epsilon}+\lambda \pi^*H_R)\cdot \xi \geq 0$
%for $\lambda >4M_2\dim X$.
%It follows that
%we may run a partial $K_{\epsilon}$-MMP, call it $\phi\colon X \dashrightarrow X'$
%which only contracts $H_R$-trivial curves
%such that for $\lambda >4M_2\dim X$ we have $\phi_*(K_{\epsilon}+\lambda \pi^*H_R)$ is nef.
%
%We may write 
%$K_{\epsilon}+\lambda \pi^*H_R = (1+\lambda)\pi^*H_R+\epsilon F = 
%(1+\lambda)(\pi^*H_R+\frac{\epsilon}{1+\lambda}F) = K_{\frac{\epsilon}{1+\lambda}}$,
%and so we see that for $\epsilon>0$ sufficiently small
%we may run a $K_{\epsilon}$-MMP which only contracts $\pi^*H_R$-trivial curves.
%
%Continuing to denote this MMP by $\phi$ we claim that we 
%may apply Theorem \ref{thm_weak_bpf} (or even just the usual basepoint
%free theorem) to
%$\frac{1}{\epsilon} \phi_*\pi^*H_R = K_{X'}+\phi_*B + \frac{1}{\epsilon}(K_{\mathcal F'}+\phi_*B_{{\rm n-inv}})$ 
%to conclude.  Indeed, by our choice of $\epsilon$, we know that this MMP is a sequence
%of steps of the $K_{\mathcal }+B_{{\rm n-inv}}$-MMP followed by a sequence of steps $K_X+B$-MMP which 
%are $K_{\mathcal }+B_{{\rm n-inv}}$-trivial.  It follows that $(K_{\mathcal F'}+\phi_*B_{{\rm n-inv}})$
%is nef and $(\mathcal F', \phi_*B_{{\rm n-inv}})$ is log canonical, and so we may apply Theorem \ref{thm_weak_bpf} (orthe classical basepoint free theorem)
%to conclude.
%\end{proof}
%\fi

